Enhancing Energy-Awareness in Deep Learning through Fine-Grained Energy Measurement

With the increasing usage, scale, and complexity of Deep Learning (DL) models, their rapidly growing energy consumption has become a critical concern. Promoting green development and energy awareness at different granularities is the need of the hour to limit carbon emissions of DL systems. However, the lack of standard and repeatable tools to accurately measure and optimize energy consumption at a fine granularity (e.g., at method level) hinders progress in this area. This paper introduces FECoM (Fine-grained Energy Consumption Meter), a framework for fine-grained DL energy consumption measurement. FECoM enables researchers and developers to profile DL APIs from energy perspective. FECoM addresses the challenges of measuring energy consumption at fine-grained level by using static instrumentation and considering various factors, including computational load and temperature stability. We assess FECoM's capability to measure fine-grained energy consumption for one of the most popular open-source DL frameworks, namely TensorFlow. Using FECoM, we also investigate the impact of parameter size and execution time on energy consumption, enriching our understanding of TensorFlow APIs' energy profiles. Furthermore, we elaborate on the considerations, issues, and challenges that one needs to consider while designing and implementing a fine-grained energy consumption measurement tool. This work will facilitate further advances in DL energy measurement and the development of energy-aware practices for DL systems.

==> appendices/evaluation_data/RQ1/combined/images-cnn/total_energy_df.tex <==
\begin{tabular}{llrrrrrrr}
 & function & run time & CPU (mean) & CPU (median) & RAM (mean) & RAM (median) & GPU (mean) & GPU (median) \\
0 & tensorflow.keras.models.Sequential.fit & 168.96 & 2038.00 & 2037.97 & -8.94 & -9.84 & 8474.62 & 7609.72 \\
1 & tensorflow.keras.models.Sequential.evaluate & 1.90 & 14.49 & 14.83 & 0.81 & 0.83 & 38.99 & 45.80 \\
2 & method-level (sum) & 170.85 & 2052.49 & 2052.80 & -8.13 & -9.01 & 8513.61 & 7655.52 \\
3 & project-level & 174.32 & 2189.51 & 2160.96 & 30.44 & 28.43 & 10314.85 & 10347.04 \\
\end{tabular}


==> sections/background.tex <==
%\assignedto{Maria}

\todiscuss{ML and DL are so common in SE papers, do we still need the following section on ML/DL?}

{\bf Machine Learning and Deep Learning.}
Machine learning (\ml{}) has been applied to solve detection, prediction, and classification problems referring to different domains (including medicine, transportation, finance, and so on).
\dl{} is a subfield of {\sc ml} that allows computational models to
use multiple processing layers
to learn representations of 
data with multiple levels
of abstraction~\cite{Lecun2015, Goodfellow2016}. 
Such data can stem from the image recognition~\cite{Krizhevsky2012, Szegedy2015},
speech recognition~\cite{Sainath2015},
and {\sc nlp}~\cite{Johnson2015} fields.
{\sc ml} and {\sc dl} models consist of two processes:
{\it training} and {\it inference}.
The {\it training} phase refers to the process of learning weights
of the internal nodes of an {\sc ml} or {\sc dl} model using training data,
to {\it learn} patterns from the data.
The {\it inference} phase refers to the process of using a trained {\sc ml} or {\sc dl} model
to make a prediction on {\it unseen} data.\todo{MK: Instead of unseen data, could we say unknown data?}

Each layer in a \dl{} model transforms the sequence of data coming
from the previous layer
or learns the representation of the input data
considering the weights of the nodes.
For example, a Convolution Neural Network ({\sc cnn})
can mimic the alternating layers of the simple and complex
cells of the visual  
cortex in data sets with animal~\cite{Felleman1991}. 
{\sc cnn}-based \dl{} models
have been proven effective for image classification,
detection~\cite{Krizhevsky2012},~\cite{Szegedy2015}
and face recognition~\cite{Lawrence1997, Parkhi2015}. 
Similarly, the Recurrent Neural Network ({\sc rnn}) and a fully-connected Neural Network
are among the various layers that can be used to compose a \dl{} model;
their arrangement within a \dl{} model is often influenced by the
problem under consideration~\cite{LAS21}.

{\bf Energy and Run-time Efficiency.}
The energy consumed by a program that uses {\sc ml} or {\sc dl} models
is measured in {\it Joules}, power required by a computer system to execute a program.
The energy consumption is calculated by the formula $E = P \times T$~\cite{iii_energy_2013}, where $P$ denotes the power consumption,
in {\it Watts}, and $T$ the total amount of time ({\it run-time performance}),
in {\it seconds}, required to execute a program.
\textit{Energy consumption} refers to the conversion of electrical energy
into thermal energy dissipated to the environment.
There are several approaches available for measuring energy consumption.
We present those approaches in detail in Section~\ref{rw}.
